Teaching Dense Retrieval Models to Specialize with Listwise Distillation and LLM Data Augmentation

While the current state-of-the-art dense retrieval models exhibit strong out-of-domain generalization, they might fail to capture nuanced domain-specific knowledge. In principle, fine-tuning these models for specialized retrieval tasks should yield higher effectiveness than relying on a one-size-fits-all model, but in practice, results can disappoint. We show that standard fine-tuning methods using an InfoNCE loss can unexpectedly degrade effectiveness rather than improve it, even for domain-specific scenarios. This holds true even when applying widely adopted techniques such as hard-negative mining and negative de-noising. To address this, we explore a training strategy that uses listwise distillation from a teacher cross-encoder, leveraging rich relevance signals to fine-tune the retriever. We further explore synthetic query generation using large language models. Through listwise distillation and training with a diverse set of queries ranging from natural user searches and factual claims to keyword-based queries, we achieve consistent effectiveness gains across multiple datasets. Our results also reveal that synthetic queries can rival human-written queries in training utility. However, we also identify limitations, particularly in the effectiveness of cross-encoder teachers as a bottleneck. We release our code and scripts to encourage further research.

==> enhancing_domain_adaptation/contrastive_comparison_table.tex <==
\begin{table}[t]
    \centering
    \adjustbox{max width=\columnwidth}{
    \begin{tabular}{l|cccc|cc|cc}
        \toprule
         & \multicolumn{4}{c}{MSMARCO} & \multicolumn{2}{c}{SciFact} & \multicolumn{2}{c}{FiQA} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
         & \multicolumn{2}{c}{DL19} & \multicolumn{2}{c}{DL20} &  &  &  &  \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         & NDCG & Recall & NDCG & Recall & NDCG & Recall & NDCG & Recall \\
        \midrule
        BGE & 70.2 & 60.9 & 67.7 & 71.5$\dagger$ & 74.1 & 96.7 & 40.6$\dagger$ & 74.2 \\
        + FT with contrastive loss & 68.6 & 61.0 & 66.8 & 70.8 & 72.1 & 96.0 & 39.5 & 70.7 \\
        + FT with listwise loss & \textbf{71.8} & \textbf{63.6} & \textbf{69.7} & 75.1 & \textbf{76.3} & \textbf{97.0} & \textbf{44.8} & \textbf{75.9}  \\
        + FT with combined loss & \textbf{71.8} & 63.0 & \textbf{69.7} & \textbf{75.5} & 76.2 & \textbf{97.0} & 44.3 & 75.8  \\
        \midrule
        GTE & \textbf{71.9} & 62.1$\dagger$ & 71.5 & 69.8$\dagger$ & 75.5 & 97.3 & 48.7 & \textbf{81.7} \\
        + FT with contrastive loss & 71.5 & 62.6 & 67.8 & 69.8 & 71.2 & 95.5 & 45.1 & 77.1 \\
        + FT with listwise loss & \textbf{72.3} & 64.7 & \textbf{72.6} & \textbf{73.8} & 75.4 & \textbf{97.7} & 48.5 & 80.2 \\
        + FT with combined loss & 71.8 & \textbf{65.6} & \textbf{72.6} & 73.3 & \textbf{76.3} & \textbf{97.7} & \textbf{49.5} & 81.4 \\
        \midrule
        Arctic & \textbf{74.4} & 64.7 & 72.1 & 74.2 & 70.5$\dagger$ & 94.8 & 42.5$\dagger$ & 74.8 \\
        + FT with contrastive loss & 72.2 & 64.3 & 71.9 & 73.1 & 69.1 & 94.9 & 41.8 & 73.0 \\
        + FT with listwise loss & \textbf{74.4} & \textbf{67.4} & \textbf{73.6} & 75.0 & 73.2 & \textbf{96.0} & 45.2 & \textbf{75.9} \\
        + FT with combined loss & 74.3 & 67.2 & \textbf{73.6} & \textbf{75.4} & \textbf{73.6} & 95.7 & \textbf{45.5} & \textbf{75.9} \\
        \midrule
        E5-unsupervised & 56.3$\dagger$ & 52.6$\dagger$ & 54.6$\dagger$ & 62.1$\dagger$ & 74.3 & \textbf{98.7} & 40.1$\dagger$ & 71.8$\dagger$ \\
        + FT with contrastive loss & 67.9 & 61.7 & 68.2 & 71.7 & 72.3 & 95.0 & 40.5 & 73.8 \\
        + FT with listwise loss & 69.9 & \textbf{63.7} & 72.7 & 74.3 & 76.2 & 96.7 & 44.0 & 75.5 \\
        + FT with combined loss & \textbf{72.4} & 63.3 & \textbf{73.2} & \textbf{75.2} & \textbf{76.3} & 97.0 & \textbf{45.4} & \textbf{77.0} \\
        \bottomrule
    \end{tabular}
    }
    \caption{NDCG@10 and Recall@100 for the original and fine-tuned (FT) models, examining the effect of the training loss. A $\dagger$ indicates a significant difference between the original and FT model with the combined loss, based on a one-sided, paired t-test $(p < 0.05)$, with Holm--Bonferroni correction across all datasets and metrics for each model's results. Best scores for each model are bolded.}
    \label{tab:loss_results}
\end{table}


==> enhancing_domain_adaptation/contrastive_threshold_tuning_figure.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\columnwidth]{contrastive_threshold_tuning.png} 
    \caption{Retrieval effectiveness scores on DL19 and DL20 at different hard negative filtering thresholds during BGE-base fine-tuning on MSMARCO passages.}
    \label{fig:threshold_tuning}
\end{figure}



==> enhancing_domain_adaptation/finetune_results.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.8}{
\begin{tabular}{l|cc|cc|cc|c}
\toprule
\textbf{Dataset} 
& \multicolumn{2}{c|}{\textbf{BGE}} 
& \multicolumn{2}{c|}{\textbf{GTE}} 
& \multicolumn{2}{c|}{\textbf{Arctic}} 
& \textbf{Promptagator} \\
& nDCG & Recall & nDCG & Recall & nDCG & Recall & nDCG \\
\midrule
DL19          
& $70.2 \;\rightarrow\; \mathbf{71.8}$ 
& $60.9 \;\rightarrow\; \mathbf{63.0}$ 
& $\mathbf{71.9} \;\rightarrow\; 71.8$ 
& $62.1 \;\rightarrow\; \mathbf{65.6}$ 
& $\mathbf{74.4} \;\rightarrow\; 74.3$ 
& $64.7 \;\rightarrow\; \mathbf{67.2}$ 
& -- \\
DL20          
& $67.7 \;\rightarrow\; \mathbf{69.7}$ 
& $71.5 \;\rightarrow\; \mathbf{75.6}$ 
& $71.5 \;\rightarrow\; \mathbf{72.6}$ 
& $69.8 \;\rightarrow\; \mathbf{72.3}$ 
& $72.1 \;\rightarrow\; \mathbf{73.6}$ 
& $74.2 \;\rightarrow\; \mathbf{75.4}$ 
& -- \\
TREC-COVID    
& $78.1 \;\rightarrow\; \mathbf{82.2}$ 
& $14.1 \;\rightarrow\; \mathbf{15.8}$
& $75.3 \;\rightarrow\; \mathbf{78.2}$
& $14.0 \;\rightarrow\; \mathbf{14.8}$
& $\mathbf{82.2} \;\rightarrow\; 80.9$
& $14.8 \;\rightarrow\; \mathbf{14.9}$
& 75.6 \\
NFCorpus      
& $37.3 \;\rightarrow\; \mathbf{38.3}$ 
& $33.7 \;\rightarrow\; \mathbf{35.8}$ 
& $35.3 \;\rightarrow\; \mathbf{37.9}$ 
& $33.1 \;\rightarrow\; \mathbf{34.6}$ 
& $36.1 \;\rightarrow\; \mathbf{37.4}$ 
& $32.4 \;\rightarrow\; \mathbf{33.7}$ 
& 33.4 \\
FiQA          
& $40.6 \;\rightarrow\; \mathbf{44.3}$ 
& $74.2 \;\rightarrow\; \mathbf{75.8}$ 
& $48.7 \;\rightarrow\; \mathbf{49.5}$ 
& $\mathbf{81.7} \;\rightarrow\; 81.4$ 
& $42.5 \;\rightarrow\; \mathbf{45.5}$ 
& $74.8 \;\rightarrow\; \mathbf{75.9}$ 
& 46.2 \\
ArguAna       
& $\mathbf{63.6} \;\rightarrow\; 61.4$ 
& $\mathbf{99.2} \;\rightarrow\; \mathbf{99.2}$ 
& $\mathbf{62.1} \;\rightarrow\; 60.9$ 
& $99.2 \;\rightarrow\; \mathbf{99.4}$ 
& $56.5 \;\rightarrow\; \mathbf{58.6}$ 
& $98.4 \;\rightarrow\; \mathbf{99.2}$ 
& 59.4 \\
Touch{\'e}-2020   
& $25.7 \;\rightarrow\; \mathbf{35.3}$ 
& $48.7 \;\rightarrow\; \mathbf{50.6}$
& $27.5 \;\rightarrow\; \mathbf{32.1}$
& $48.3 \;\rightarrow\; \mathbf{49.0}$
& $33.2 \;\rightarrow\; \mathbf{37.9}$
& $50.0 \;\rightarrow\; \mathbf{52.4}$
& 34.5 \\
DBPedia       
& $40.7 \;\rightarrow\; \mathbf{45.5}$ 
& $53.0 \;\rightarrow\; \mathbf{56.3}$ 
& $36.9 \;\rightarrow\; \mathbf{44.7}$ 
& $46.9 \;\rightarrow\; \mathbf{55.2}$ 
& $44.7 \;\rightarrow\; \mathbf{45.1}$ 
& $\mathbf{58.7} \;\rightarrow\; 57.2$ 
& 38.0 \\
SCIDOCS       
& $\mathbf{21.7} \;\rightarrow\; 19.4$ 
& $\mathbf{49.6} \;\rightarrow\; 45.5$ 
& $\mathbf{21.7} \;\rightarrow\; 20.2$ 
& $\mathbf{50.1} \;\rightarrow\; 46.6$ 
& $\mathbf{20.0} \;\rightarrow\; 18.6$ 
& $42.3 \;\rightarrow\; \mathbf{43.5}$
& 18.4 \\
FEVER         
& $\mathbf{86.3} \;\rightarrow\; 80.0$ 
& $\mathbf{97.2} \;\rightarrow\; 95.7$ 
& $\mathbf{92.1} \;\rightarrow\; 82.4$ 
& $\mathbf{97.5} \;\rightarrow\; 96.0$ 
& $\mathbf{85.6} \;\rightarrow\; 80.4$ 
& $\mathbf{97.6} \;\rightarrow\; 96.1$ 
& 77.0 \\
Climate-FEVER 
& $\mathbf{31.2} \;\rightarrow\; 25.1$ 
& $\mathbf{63.6} \;\rightarrow\; 59.3$ 
& $\mathbf{40.1} \;\rightarrow\; 30.3$ 
& $\mathbf{71.7} \;\rightarrow\; 63.8$ 
& $\mathbf{34.7} \;\rightarrow\; 27.2$ 
& $\mathbf{66.7} \;\rightarrow\; 63.1$ 
& 16.8 \\
SciFact       
& $74.1 \;\rightarrow\; \mathbf{76.2}$ 
& $96.7 \;\rightarrow\; \mathbf{97.0}$ 
& $75.5 \;\rightarrow\; \mathbf{76.3}$ 
& $97.3 \;\rightarrow\; \mathbf{97.7}$ 
& $70.5 \;\rightarrow\; \mathbf{73.6}$ 
& $94.8 \;\rightarrow\; \mathbf{95.7}$ 
& 65.0 \\
\bottomrule
\end{tabular}
}
\caption{nDCG@10 and Recall@100 for the models (before fine-tuning 
$\rightarrow$ after fine-tuning). Bolded values indicate the best score for each model on each dataset. Promptagator scores 
(nDCG only) are shown on the right for reference.}
\label{tab:full_training}
\end{table*}

==> enhancing_domain_adaptation/query_quality.tex <==
\begin{table}[t]
    \centering
    \adjustbox{max width=\columnwidth}{
    \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}{Query Type} & \multirow{2}{*}{\# Queries} & \multicolumn{2}{c}{DL19} & \multicolumn{2}{c}{DL20} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
         & & NDCG & Recall & NDCG & Recall \\
        \midrule
        (No fine-tuning) & - & 56.3 & 52.6 & 54.6 & 62.1 \\
        \midrule
        User Queries (Human)             & 56K    & 71.6 & 63.9 & \textbf{73.4} & 73.0 \\
        User Queries Few-Shot (Synthetic)& 56K    & 71.7 & 64.9 & 70.3 & 72.1 \\
        User Queries Few-Shot (Synthetic)& 96K    & 72.8 & \textbf{65.3} & 72.8 & \textbf{74.5} \\
        User Queries Zero-shot (Synthetic)        & 56K    & 70.8 & 62.2 & 70.5 & 73.1 \\
        User Queries Zero-shot (Synthetic)        & 98K    & \textbf{74.0} & 62.9 & 71.8 & 73.7 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Retrieval effectiveness for the E5-unsupervised model fine-tuned with human-written and synthetic queries. For the synthetic queries, results are provided for both a subset of 56K queries to provide a fair comparison and the full query set.}
    \label{tab:query_quality}
\end{table}


==> enhancing_domain_adaptation/rerank_bge.tex <==
\begin{table}[t]
\centering
\adjustbox{max width=0.6\columnwidth}{
\begin{tabular}{l|cc}
\toprule
\textbf{Dataset} & \textbf{BGE} & \textbf{RankT5-3B} \\
\midrule
DL19            & 70.2          & \textbf{75.1} \\
DL20            & 67.7          & \textbf{77.2} \\
TREC-COVID      & 78.1          & \textbf{85.7} \\
NFCorpus        & 37.3          & \textbf{40.4} \\
FiQA            & 40.6          & \textbf{52.6} \\
SCIDOCS         & \textbf{21.7} & 19.3 \\
ArguAna         & \textbf{63.6} & 34.9 \\
Touché-2020     & 25.7          & \textbf{38.6} \\
DBPedia         & 40.7          & \textbf{48.1} \\
FEVER           & \textbf{86.3} & 84.9 \\
Climate-FEVER   & \textbf{31.2} & 27.3 \\
SciFact         & 74.1          & \textbf{77.1} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{NDCG@10} Scores for BGE and RankT5-3B reranking the top-100 BGE retrieved passages. Best scores are bolded.}
\label{tab:rerank_ndcg}
\end{table}


==> enhancing_domain_adaptation/specific_queries.tex <==
\begin{table}[t]
    \centering
    \adjustbox{max width=\columnwidth}{
    \begin{tabular}{l c c c | c c c c}
        \toprule
        \textbf{Query Type} 
            & \multicolumn{3}{c}{\textbf{\#Q}} 
            & \multicolumn{4}{c}{\textbf{NDCG@10}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-8}
        & (DL19+20) & FiQA & Sci
        & DL19 & DL20 & FiQA & SciFact \\
        \midrule
        (No fine-tuning)
            & -- & -- & --
            & 56.3 & 54.6 & 40.1 & 74.4 \\
        \midrule
        {MSMARCO User Queries} 
            & 96K & 39k & 5k 
            & 72.8 & 72.8 & 43.7 & 75.2 \\
        {Claims} 
            & 136k & 46k & 5k 
            & 65.3 & 68.0 & 40.7 & 74.5 \\
        {Titles} 
            & 99k & 34k & 5k 
            & \textbf{72.9} & 71.6 & 42.9 & 72.3 \\
        {All Queries} 
            & 646k & 240k & 30k 
            & 72.4 & \textbf{73.2} & \textbf{45.4} & \textbf{76.3} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Retrieval effectiveness when training the E5-unsupervised model with different query types and all generated queries. \#Q gives the number of queries for training.}
    \label{tab:query_type}
\end{table}

